Large-scale Interstellar Structure and the Heliosphere

The properties of interstellar clouds near the Sun are ordered by the Loop I superbubble and by the interstellar radiation field. Comparisons of the kinematics and magnetic field of the interstellar gas flowing past the Sun, including the Local Interstellar Cloud (LIC), indicate a geometric relation between Loop I as defined by radio synchrotron emission, and the interstellar magnetic field that polarizes nearby starlight. Depletion of Fe and Mg onto dust grains in the LIC shows a surprising relation to the far ultraviolet interstellar radiation field that is best explained by a scenario for the LIC to be extended, possibly filamentary, porous material drifting through space with the Loop I superbubble. The interstellar velocity and magnetic field measured by the Interstellar Boundary Explorer (IBEX) help anchor our understanding of the physical properties of the nearby interstellar medium.

==> aspauthor.tex <==
% This is the aspauthor.tex LaTeX file
% Copyright 2010, Astronomical Society of the Pacific Conference Series

%\documentclass[11pt,twoside]{article}
%\usepackage{./asp2010}

\resetcounters

\bibliographystyle{asp2010}

\markboth{Author1, Author2, and Author3}{Author's Final Checklist}

%\begin{document}

\title{ASP Author Template}
\author{Sample~Author1,$^1$ Sample~Author2,$^2$ and Sample~Author3$^3$
\affil{$^1$Institution Full Address for Author1}
\affil{$^2$Institution Full Address for Author2}
\affil{$^3$Institution Full Address for Author3}}

\begin{abstract}
This is the Astronomical Society of the Pacific (ASP) 2010 author template file.  This sample author template includes the ASP author checklist.
\end{abstract}

\section{The Template}
To fill in this template, make sure that you read and follow the ASPCS Instructions for Authors and Editors available for download online.  Hints and tips for including graphics, tables, citations, and other formatting helps are available there.

\subsection{The Author Checklist}
The following checklist should be followed when writing a submission to a conference proceedings to be published by the ASP.

\begin{itemize}
\checklistitemize
\item Article is within page limitations set by editor. 
\item Paper compiles properly without errors or warnings.
\item No fundamental modifications to the basic template are present, including special definitions, special macros, packages, \verb"\vspace" commands, font adjustments, etc. %(§ 3.3, p. 10)
\item Commented-out text has been removed. %(§ 3.3, p. 10,11)
\item Author and shortened title running heads are proper for the paper and shortened so page number is within the margin. %(§ 3.1, p. 4)
\item Paper checked for general questions of format and style, including, but not limited to, the following:
\begin{itemize}
  \item capitalization, layout, and length of running heads, titles  and \\sections/subsections;  % (§ 3.1, p. 4) (§ 3.2, p. 5) (§ 3.3, p. 8)
  \item page numbers within margin; % (§ 3.1, p. 4)
  \item author names spelled correctly and full postal addresses given; % (§ 3.2, p. 5-6)
  \item abstracts; % (§ 3.2, p. 7);
  \item all margins---left, right, top and bottom; % (§3.1, p. 4; §3.2, p. 5; §3.3, p. 9; §3.6, p. 21);
  \item standard font size and no Type 3 fonts; %(§ 3.3, pp. 10-11; § 3.6, p. 23; § 4.2, p. 25);
  \item spacing; % (§ 3.3, pp. 9-10);
  \item section headings. % (§ 3.3; p. 8).
\end{itemize}
\item All tables are correctly positioned within margins, are properly formatted, and are referred to in the text.  %(§ 3.5, pp. 16-20)
\item All figures are correctly positioned within margins, are minimum 300 dpi resolution, not too dark or too light, do not contain embedded fonts, and are referred to in the text.  All labeling or text will be legible with 10\% reduction.  Questionable images printed, checked and replaced if necessary.  Figures do not cover text or running heads, and proper permissions have been granted and acknowledged.  %(§ 3.6, pp. 21-24)
\item All acknowledgments and discussions are in proper format.  % (pp. 11-12, p. 20)
\item If there are acknowledgments at the end of the article, ensure that the author has used
the \verb"\acknowledgments" command and not the commands
\\ \verb"\begin{Acknowledgments}", \verb"\end{Acknowledgments}".
Acknowledgments should only be used for thanking institutions,
groups, and individuals who have directly contributed to the work.
\item All references quoted in the text are listed in the bibliography; all items in the bibliography have been referred to in the text.  % (§ 4, pp. 24-28)
\item All bibliography entries are in the proper format, using one of the referencing styles given. Each of the references is bibliographically complete, including full names of authors, editors, publishers, place of publication, page numbers, years, etc. % (§§ 4.2-4.3, pp. 25-28)
\item A complete Bib\TeX\ file is ready to submit to the editor.
\item References to preprints replaced with publication information when possible.
\end{itemize}

\acknowledgements The ASP would like to the thank the dedicated researchers that are publishing with the ASP.

\bibliography{editor}

%\end{document}

